Empirically explaining SGD from a line search perspective

Optimization in Deep Learning is mainly guided by vague intuitions and strong assumptions, with a limited understanding how and why these work in practice. To shed more light on this, our work provides some deeper understandings of how SGD behaves by empirically analyzing the trajectory taken by SGD from a line search perspective. Specifically, a costly quantitative analysis of the full-batch loss along SGD trajectories from common used models trained on a subset of CIFAR-10 is performed. Our core results include that the full-batch loss along lines in update step direction is highly parabolically. Further on, we show that there exists a learning rate with which SGD always performs almost exact line searches on the full-batch loss. Finally, we provide a different perspective why increasing the batch size has almost the same effect as decreasing the learning rate by the same factor.

==> line_analysis/figure3_similarity_matrices_res_net18.tex <==


\begin{figure}[h!]
	\centering
	\def\scale{0.4}
	\begin{tabular}{ c c c}
		
		
		
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom0_resnet18_augment_result/statistics_plots/distance_matrix_first_50.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom0_resnet18_augment_result/statistics_plots/distance_matrix_after_line50.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom0_resnet18_augment_result/statistics_plots/consecutive_line_distances.pgf"}}\\
		
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/distance_matrix_first_50.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/distance_matrix_after_line50.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/consecutive_line_distances.pgf"}}
	\end{tabular}
	\caption{\textbf{ResNet-18:} Distances of the shape of full-batch losses along lines in a window of 0.2 around the minimum.
		\textbf{Row 1:} SGD without momentum. \textbf{Row 2:} SGD with momentum. Since the offset is not of interest the minimum is shifted to 0. The distances are rather high for the first 10 lines (left). For the following lines they are less then 0.3 MAE (middle). The MAE of losses along consecutive lines are given on the right.}
	\label{la_fig_similarity_matrices_res_net18}
\end{figure}

==> line_analysis/figure_batch_size_metrics_mobilenet_mom_09.tex <==
\begin{figure}[b!]
	\centering
	\def\scale{0.36}
	\begin{tabular}{ c c}
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_distances_step_accumulated.pgf"}}&	
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_distances_step_accumulated.pgf"}}&
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_distances_step_accumulated.pgf"}}\\
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots//CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_improvements_step_accumulated.pgf"}}&\hspace{0.1cm}	
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_improvements_step_accumulated.pgf"}}\\
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_improvements_step_accumulated.pgf"}}
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/directional_derivatives.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/directional_derivatives_ratio.pgf"}}
	\end{tabular}\\
	\caption{\textbf{Row 1} Comparing the influence of the batch size on the loss improvement. Left: SGD with the original learning rate of 0.1. Right: parabolic approximation line search (PAL).
		\textbf{Row 2: } Analysis of the relation of the batch size to the absolute directional derivative (=gradient norm) which shows in detail that increasing the batch size has a similar effect as decreasing the learning rate by the same factor.  \textbf{e.r.}  stands for expected ratio.}.
	\label{la_fig_distances_batchwise}
\end{figure}


%\begin{figure}[h!]
%	\centering
%		\def\scale{0.45}
%	\def\basis{10e-5}
%	\begin{tabular}{ c c c }
%				
%
%		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/directional_curvatures.pgf"}}
%\end{tabular}
%
%	\caption{TODO}
%	mobile_net{fig:_improvements_batchwise}
%\end{figure}



%\begin{figure}[h!]
%	\centering
%	
%	%\scalebox{1.0}{
%	%\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
%
%
%
%%	\scalebox{0.55}{
%%
%%		\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/directional_curvature_ratio.pgf"}\hspace{-0.1cm}
%%		\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/fb_min_step_ratio_batches.pgf"}\hspace{-0.1cm}
%%	}
%	\normalsize
%	\caption{Todo}
%	mobile_net{fig:_directional_derivatives_and_curvatures}
%\end{figure}



%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex

==> line_analysis/figure_batch_size_metrics_momentum.tex <==
\begin{figure}[t!]

	\centering
		\def\scale{0.4}
	%\vspace{-0.5cm}
	\begin{tabular}{ c c}
	
			%\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_distances_step_accumulated.pgf"}}&
			%\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_distances_step_accumulated.pgf"}}&
		%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_distances_step_accumulated.pgf"}\hspace{-0.1cm}
			%\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_distances_step_accumulated.pgf"}}\\

			%\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_improvements_step_accumulated.pgf"}}&
			%\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_improvements_step_accumulated.pgf"}}\\
		%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_improvements_step_accumulated.pgf"}\hspace{-0.1cm}
			%\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_improvements_step_accumulated.pgf"}}\\
			\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/directional_derivatives.pgf"}}&
			\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet20_augment_result/statistics_plots/batch_size_comparison/directional_derivatives_ratio.pgf"}}
	\end{tabular}
	\vspace{-0.4cm}
	\caption{Analyzing the effect of different batch sizes on \textbf{SGD training with momentum 0.9.} For explanations see Figure \ref{la_fig_distances_batchwise}.}
	\label{la_fig_distances_batchwise_momentum}
\end{figure}


%\begin{figure}[h!]
%	\centering
%
%	
%	\scalebox{0.45}{				
%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/directional_derivatives.pgf"}\hspace{-0.1cm}	
%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/directional_derivatives_ratio.pgf"}
%		%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/directional_curvatures.pgf"}\hspace{-0.1cm}	
%	}
%	\normalsize
%	\caption{TODO}
%	mobile_net{fig:_improvements_batchwise_momentum}
%\end{figure}



%\begin{figure}[h!]
%	\centering
%	
%	%\scalebox{1.0}{
%	%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
%
%
%
%%	\scalebox{0.55}{
%%
%%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/directional_curvature_ratio.pgf"}\hspace{-0.1cm}
%%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/fb_min_step_ratio_batches.pgf"}\hspace{-0.1cm}
%%	}
%	\normalsize
%	\caption{Todo}
%	mobile_net{fig:_directional_derivatives_and_curvatures}
%\end{figure}



%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex

==> line_analysis/figure_batch_size_metrics_res_net_18_mom_09.tex <==
\begin{figure}[b!]
	\centering
	\def\scale{0.36}
	\begin{tabular}{ c c}
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_distances_step_accumulated.pgf"}}&	
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_distances_step_accumulated.pgf"}}&
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_distances_step_accumulated.pgf"}}\\
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots//CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_improvements_step_accumulated.pgf"}}&\hspace{0.1cm}	
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_improvements_step_accumulated.pgf"}}\\
		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_improvements_step_accumulated.pgf"}}
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/directional_derivatives.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/batch_size_comparison/directional_derivatives_ratio.pgf"}}
	\end{tabular}\\
	\caption{\textbf{Row 1} Comparing the influence of the batch size on the loss improvement. Left: SGD with the original learning rate of 0.1. Right: parabolic approximation line search (PAL).
		\textbf{Row 2: } Analysis of the relation of the batch size to the absolute directional derivative (=gradient norm) which shows in detail that increasing the batch size has a similar effect as decreasing the learning rate by the same factor.  \textbf{e.r.}  stands for expected ratio.}.
	\label{la_fig_distances_batchwise}
\end{figure}


%\begin{figure}[h!]
%	\centering
%		\def\scale{0.45}
%	\def\basis{10e-5}
%	\begin{tabular}{ c c c }
%				
%
%		%\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/directional_curvatures.pgf"}}
%\end{tabular}
%
%	\caption{TODO}
%	mobile_net{fig:_improvements_batchwise}
%\end{figure}



%\begin{figure}[h!]
%	\centering
%	
%	%\scalebox{1.0}{
%	%\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
%
%
%
%%	\scalebox{0.55}{
%%
%%		\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/directional_curvature_ratio.pgf"}\hspace{-0.1cm}
%%		\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet20_augment_result/statistics_plots/fb_min_step_ratio_batches.pgf"}\hspace{-0.1cm}
%%	}
%	\normalsize
%	\caption{Todo}
%	mobile_net{fig:_directional_derivatives_and_curvatures}
%\end{figure}



%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex

==> line_analysis/figure_batch_size_metrics_res_net_18_momentum.tex <==
\begin{figure}[b!]
	\vspace{-3cm}
	\centering
	\def\scale{0.4}
	\begin{tabular}{ c c c}
		
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_distances_step_accumulated.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_distances_step_accumulated.pgf"}}&
		%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_distances_step_accumulated.pgf"}\hspace{-0.1cm}
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_distances_step_accumulated.pgf"}}\\
		
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_improvements_step_accumulated.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/PALmu=0,1_improvements_step_accumulated.pgf"}}&
		%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/SGD(original)lambda=0,1_improvements_step_accumulated.pgf"}\hspace{-0.1cm}
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/batch_size_comparison/FBPAL&SGDmu=0,1_improvements_step_accumulated.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/directional_derivatives.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/directional_derivatives_ratio.pgf"}}&
	\end{tabular}
	
	\caption{\textbf{SGD training process with momentum 0.9 on ResNet-18} \textbf{Row 1 and 2: } Comparing the influence of the batch size on several update step strategies: 1. SGD with the original learning rate of 0.1. 2. parabolic approximation line search (PAL). 3. Our proposed FBPAL\&SGD which still performs well on low batch sizes.
		\textbf{Row 3: } Analysis of the relation of batch size and directional derivative (= negative gradient norm).  For batch sizes between 64 and 256 directional derivatives behave almost proportional to the batch size.}
	\label{la_fig_distances_batchwise_momentum_res_net18}
\end{figure}


%\begin{figure}[h!]
%	\centering
%
%	
%	\scalebox{0.45}{				
%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/directional_derivatives.pgf"}\hspace{-0.1cm}	
%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/directional_derivatives_ratio.pgf"}
%		%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/directional_curvatures.pgf"}\hspace{-0.1cm}	
%	}
%	\normalsize
%	\caption{TODO}
%	mobile_net{fig:_improvements_batchwise_momentum}
%\end{figure}



%\begin{figure}[h!]
%	\centering
%	
%	%\scalebox{1.0}{
%	%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/distance_matrix.pgf"}}\\
%
%
%
%%	\scalebox{0.55}{
%%
%%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/directional_curvature_ratio.pgf"}\hspace{-0.1cm}
%%		\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/fb_min_step_ratio_batches.pgf"}\hspace{-0.1cm}
%%	}
%	\normalsize
%	\caption{Todo}
%	mobile_net{fig:_directional_derivatives_and_curvatures}
%\end{figure}



%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex

==> line_analysis/figure_polynomial_approximations_mobilenet_mom_09.tex <==

\begin{figure}[t!]
	\centering
	\def\scale{0.37}
	\begin{tabular}{ c c c}
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_mobilenet_result/statistics_plots/mae_of_polynomial_fit_of_degree_1.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_mobilenet_result/statistics_plots/mae_of_polynomial_fit_of_degree_2.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_mobilenet_result/statistics_plots/coefficients_of_polynomial_fit_of_degree_2.pgf"}}\\
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_mobilenet_result/statistics_plots/mae_of_polynomial_fit_of_degree_1.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_mobilenet_result/statistics_plots/mae_of_polynomial_fit_of_degree_2.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_mobilenet_result/statistics_plots/coefficients_of_polynomial_fit_of_degree_2.pgf"}}
	\end{tabular}
	\caption{MAE of polynomial approximations of the full-batch loss of degree 1 and 2. \textbf{Row 1:} SGD without momentum. \textbf{Row 2:} SGD with momentum. Full-batch losses along lines can be well fitted by polynomials of degree 2. The slope of the approximation stays roughly constant whereas the curvature decreases.}
	\label{la_fig_polynomial_approximations}
\end{figure}


==> line_analysis/figure_polynomial_approximations_mom.tex <==
\begin{figure}[h!]
\centering
\large
%\scalebox{1.0}{
%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
\scalebox{0.6}{
\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/mae_of_polynomial_fit_of_degree_1.pgf"}
\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/mae_of_polynomial_fit_of_degree_2.pgf"}
\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/coefficients_of_polynomial_fit_of_degree_2.pgf"}
}

\normalsize
\caption{(Momentum) MAE of polynomial approximations of degree 1 and 2. Line Losses can be well fitted by polynomials of degree 2. The slope stays roughly constant whereas the curvature increases.}
\label{la_fig_polynomial_approximations_mom}
\end{figure}

==> line_analysis/figure_polynomial_approximations_res_net_18_mom_09.tex <==

\begin{figure}[h!]
	\centering
	\def\scale{0.37}
	\begin{tabular}{ c c c}
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet18_augment_result/statistics_plots/mae_of_polynomial_fit_of_degree_1.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet18_augment_result/statistics_plots/mae_of_polynomial_fit_of_degree_2.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet18_augment_result/statistics_plots/coefficients_of_polynomial_fit_of_degree_2.pgf"}}\\
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet18_augment_result/statistics_plots/mae_of_polynomial_fit_of_degree_1.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet18_augment_result/statistics_plots/mae_of_polynomial_fit_of_degree_2.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet18_augment_result/statistics_plots/coefficients_of_polynomial_fit_of_degree_2.pgf"}}
	\end{tabular}
	\caption{MAE of polynomial approximations of the full-batch loss of degree 1 and 2. \textbf{Row 1:} SGD without momentum. \textbf{Row 2:} SGD with momentum. Full-batch losses along lines can be well fitted by polynomials of degree 2. The slope of the approximation stays roughly constant whereas the curvature decreases.}
	\label{la_fig_polynomial_approximations}
\end{figure}


==> line_analysis/figure_similarity_matrices_mobilenet_mom_09.tex <==


\begin{figure}[h!]
	\centering
	\def\scale{0.365}
	\begin{tabular}{ c c c}
		
		
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_mobilenet_result/statistics_plots/distance_matrix_first_50.pgf"}}&
		\scalebox{\scale}{\hspace{-0.8cm}\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_mobilenet_result/statistics_plots/distance_matrix_after_line50.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_mobilenet_result/statistics_plots/consecutive_line_distances.pgf"}}\\
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_mobilenet_result/statistics_plots/distance_matrix_first_50.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_mobilenet_result/statistics_plots/distance_matrix_after_line50.pgf"}}& 
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_mobilenet_result/statistics_plots/consecutive_line_distances.pgf"}}
	\end{tabular}
	\caption{Distances of the shape of full-batch losses along lines in a window around the current position $s=0$.
		\textbf{Row 1:} SGD without momentum. \textbf{Row 2:} SGD with momentum. Since the offset is not of interest the minimum is shifted to 0 on the y-axis. The distances are rather high for the first 10 lines (left). For the following lines the distances are less then 0.3 MAE (middle) and concentrate around 0.01. The MAEs of the full-batch loss of pairs of consecutive lines are given on the right.}
	\label{la_fig_similarity_matrices}
\end{figure}

==> line_analysis/figure_similarity_matrices_mom.tex <==


\begin{figure}[h!]
\centering
\large
%\scalebox{1.0}{
%\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
\scalebox{0.45}{
\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/distance_matrix_first_50.pgf"}
\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/distance_matrix_after_line50.pgf"}
\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/statistics_plots/consecutive_line_distances.pgf"}
}


\normalsize
\caption{(Momentum) Distances of the shape full batch losses along lines in a window of 0.2 around the minimum. Since the offset is not of interest the minimum is shifted to 0. The distances are rather high for the first 15 lines (left). For the following lines they are less then 0.3 MAE.The distances of consecutive line losses are given on the right. (Loss along lines of a ResNet-20 trained on 8\% of CIFAR-10 with SGDM.) TODO momenutm plots in appendix}
\label{la_fig_similarity_matrices_mom}
\end{figure}

==> line_analysis/figure_similarity_matrices_res_net_18_mom_09.tex <==


\begin{figure}[h!]
	\centering
	\def\scale{0.365}
	\begin{tabular}{ c c c}
		
		
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet18_augment_result/statistics_plots/distance_matrix_first_50.pgf"}}&
		\scalebox{\scale}{\hspace{-0.8cm}\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet18_augment_result/statistics_plots/distance_matrix_after_line50.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom0_resnet18_augment_result/statistics_plots/consecutive_line_distances.pgf"}}\\
		
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet18_augment_result/statistics_plots/distance_matrix_first_50.pgf"}}&
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet18_augment_result/statistics_plots/distance_matrix_after_line50.pgf"}}& 
		\scalebox{\scale}{\input{"line_analysis/figure_data/line_plots/CIFAR10_mom09_resnet18_augment_result/statistics_plots/consecutive_line_distances.pgf"}}
	\end{tabular}
	\caption{Distances of the shape of full-batch losses along lines in a window around the current position $s=0$.
		\textbf{Row 1:} SGD without momentum. \textbf{Row 2:} SGD with momentum. Since the offset is not of interest the minimum is shifted to 0 on the y-axis. The distances are rather high for the first 10 lines (left). For the following lines the distances are less then 0.3 MAE (middle) and concentrate around 0.01. The MAEs of the full-batch loss of pairs of consecutive lines are given on the right.}
	\label{la_fig_similarity_matrices}
\end{figure}

==> line_analysis/figure_strategy_metrics_res_net_18_momentum.tex <==
\begin{figure}[h!]
	\centering
	\def\scale{0.4}
	\def\basis{10e-5}
	\begin{tabular}{ c c c }
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/step_step.pgf"}}&
		%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library	
		\pgfplotsset
		{
			y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
			y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},	
		}
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/distances_step.pgf"}}&
		\pgfplotsset
		{
			y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
			y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},	
		}
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/improvements_step.pgf"}}\\
		
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/distances_step_accumulated.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/improvements_step_accumulated.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet18_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/fb_min_step_ratio.pgf"}}
	\end{tabular}
	\caption{\textbf{SGD training process with momentum 0.9 on ResNet-18}. Several metrics to compare update step strategies: 1. the performed update steps, 2. the distance to the minimum of the full batch loss ($s_{opt}-s_{upd}$), which is the optimal update step from a local perspective. 3. the loss improvement per step given  as:  $l(0)-l(s_{upd}))$ where $s_{upd}$ is the update step of a strategy. Average smoothing with a kernel size of 25 is applied. }
	\label{la_fig_strategy_metrics_momentum_res_net}
\end{figure}

%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex
